Stochastic Control Barrier Functions for Economics

Control barrier functions (CBFs) and safety-critical control have seen a rapid increase in popularity in recent years, predominantly applied to systems in aerospace, robotics and neural network controllers. Control barrier functions can provide a computationally efficient method to monitor arbitrary primary controllers and enforce state constraints to ensure overall system safety. One area that has yet to take advantage of the benefits offered by CBFs is the field of finance and economics. This manuscript re-introduces three applications of traditional control to economics, and develops and implements CBFs for such problems. We consider the problem of optimal advertising for the deterministic and stochastic case and Merton's portfolio optimization problem. Numerical simulations are used to demonstrate the effectiveness of using traditional control solutions in tandem with CBFs and stochastic CBFs to solve such problems in the presence of state constraints.

==> sections/Limitations.tex <==
\section{Limitations}

The proposed method has clear limitations that must be directly addressed. Firstly, this formulation relies on a nonlinear solver to obtain a control solution that satisfies the constraints. Nonlinear solvers are in general not complete, and take longer to find a solution. Secondly, the derivative of the constraint, $\dot{h}(\boldsymbol{x}, \boldsymbol{u})$, is of course an approximation using this method. One can imagine that for excessively large timesteps, this formulation may no longer ensure safety as the constraint may be satisfied at points $\boldsymbol{x}_t$ and $\boldsymbol{x}_{t + \Delta t}$ but not along the trajectory between these points. For example, the system may be safe at two states outside of an obstacle, but the trajectory between these points may pass through the obstacle. 

However, there are some cases where the proposed approach may actually outperform traditional approaches for large timesteps. Consider a simple example of a maximum speed constraint imposed on an autonomous robot, and say that this robot must run its control system and safety enforcement system at a low frequency due to outdated hardware or computationally expensive algorithms. In a case where the desired controller attempts to quickly increase the speed of the robot, it will quickly approach the boundary of the safe set. In the case of enforcing safety with a classical CBF approach (i.e. using the instantaneous tangent velocity of $h(x)$), when operating at a high frequency the CBF can quickly react over multiple timesteps to prevent a safety violation. When operating at a low frequency, the CBF may ensure safety at one point in time, but by the time the next gradient computation is performed, safety may already be violated. It is possible that safety will not be ensured because the safety condition is only checked \textit{before} the violation occurs. The formulation presented in this paper, on the other hand, takes into account the forward projection over that longer timestep, making it possible to ensure safety for longer timesteps. In this case, the timestep is taken into account when determining $\boldsymbol{u}_{\rm act}$. This longer timestep allows the NLP to be used more readily, as it provides more time for the solution to be obtained.
% It is straightforward to imagine a case where the controller will violate this constraint, 
% \hl{However,.... blah give example for when large timesteps could actually be good and traditional approach may fail.}

The authors believe that these limitations are not overly prohibitive. This method allows anyone with minimal CBF experience to implement a safety filter on an already existing dynamical system and controller set. The computational and mathematical burden is transferred to the NLP and the numerical integrator of choice, which can be very advantageous.
% \\
% (briefly explain how this is a very easy method to get going, you only need to be able to integrate your dynamics, which can be done by integrators with high fidelity)

